Atlas: Multi-Scale Attention Improves Long Context Image Modeling

Efficiently modeling massive images is a long-standing challenge in machine learning. To this end, we introduce Multi-Scale Attention (MSA). MSA relies on two key ideas, (i) multi-scale representations (ii) bi-directional cross-scale communication. MSA creates O(log N) scales to represent the image across progressively coarser features and leverages cross-attention to propagate information across scales. We then introduce Atlas, a novel neural network architecture based on MSA. We demonstrate that Atlas significantly improves the compute-performance tradeoff of long-context image modeling in a high-resolution variant of ImageNet 100. At 1024px resolution, Atlas-B achieves 91.04% accuracy, comparable to ConvNext-B (91.92%) while being 4.3x faster. Atlas is 2.95x faster and 7.38% better than FasterViT, 2.25x faster and 4.96% better than LongViT. In comparisons against MambaVision-S, we find Atlas-S achieves 5%, 16% and 32% higher accuracy at 1024px, 2048px and 4096px respectively, while obtaining similar runtimes. Code for reproducing our experiments and pretrained models is available at https://github.com/yalalab/atlas.

==> sections/experiments/block_composition.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{10pt} % Adjust column spacing
\renewcommand{\arraystretch}{1.2} % Adjust row spacing
\caption{Block-level comparison of different attention mechanisms.}
\label{tab:block-comparison}
\begin{tabular}{l|cc}
    \toprule
    \textbf{Block} & \textbf{Runtime (min)} & \textbf{Top-1 (\%)} \\
    \midrule
    MSA (Atlas) & 80 & 77.34 \\
    Hierarchical Attention (FasterViT) & 78 & 53.65 \\
    LongViT & 154 & 61.09 \\
    ViT & 81 & 72.54 \\
    MambaVision (window size=8) & 68 & 47.26 \\
    MambaVision (window size=16) & 59 & 62.69 \\
    WViT (window size=8) & 45 & 62.69 \\
    WViT (window size=16) & 44 & 66.82 \\
    \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{10pt} 
\renewcommand{\arraystretch}{1.2} 
\caption{Comparison of different composition strategies.}
\label{tab:composition-comparison}
\begin{tabular}{l|c}
    \toprule
    \textbf{Composition} & \textbf{Top-1 (\%)} \\
    \midrule
    Stack & 69.88 \\
    Downsample (Conv) & 56.14 \\
    Atlas (D2D10) & 70.09 \\
    \bottomrule
\end{tabular}
\end{table*}

% \begin{table*}
%     \begin{tabular}{l|cc}
%         \toprule
%         Block & Runtime(m) & Top-1 \\
%         MSA (atlas) & 80 & 77.344 \\
%         Hierarchical Attention (fastervit) & 78 & 53.65 \\
%         longvit & 154 & 61.09 \\
%         vit & 81 & 72.54 \\
%         mambavison (windowsize=8) & 68 & 47.26 \\
%         mambavison (windowsize=16) & 59 & 62.69 \\
%         wvit (windowsize=8) & 45 & 62.69 \\
%         wvit (windowsize=16) & 44 & 66.82 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Block-level comparison of different attention mechanisms.}
% \end{table*}

% \begin{table*}
%     \begin{tabular}{l|cc}
%         \toprule
%         Composition & Top-1 \\
%         \midrule
%         Stack & 69.88 \\
%         downsample (conv) & 56.14 \\
%         atlas (d2d10) & 70.09 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Composition strategy comparison}
% \end{table*}

